There is a Time and Place for Reasoning Beyond the Image

Images are often more significant than only the pixels to human eyes, as we can infer, associate, and reason with contextual information from other sources to establish a more complete picture. For example, in Figure 1, we can find a way to identify the news articles related to the picture through segment-wise understandings of the signs, the buildings, the crowds, and more. This reasoning could provide the time and place the image was taken, which will help us in subsequent tasks, such as automatic storyline construction, correction of image source in intended effect photographs, and upper-stream processing such as image clustering for certain location or time. In this work, we formulate this problem and introduce TARA: a dataset with 16k images with their associated news, time, and location, automatically extracted from New York Times, and an additional 61k examples as distant supervision from WIT. On top of the extractions, we present a crowdsourced subset in which we believe it is possible to find the images' spatio-temporal information for evaluation purpose. We show that there exists a $70\%$ gap between a state-of-the-art joint model and human performance, which is slightly filled by our proposed model that uses segment-wise reasoning, motivating higher-level vision-language joint models that can conduct open-ended reasoning with world knowledge. The data and code are publicly available at https://github.com/zeyofu/TARA.

==> files/results_seg.tex <==

\begin{table}[t]
\small
\centering
\setlength{\tabcolsep}{4pt}
\begin{tabular}{c|cc}
\toprule
Model & Accuracy & Example-F1
\\ \midrule
CLIP & 11.11 & 44.96 \\
CLIP+ & 15.72 & 49.74 \\
CLIP+WIT & 11.11 & 45.20 \\
CLIP+Seg & \textbf{16.46} & \textbf{50.52} \\
\midrule
Human & 86.21 & 92.41 \\
\bottomrule
\end{tabular}
\vspace{-0.5em}\caption{Summary of the performance for different baselines on the image location prediction. Accuracy does not consider hierarchies and Example-F1 considers hierarchies.(\%)}
\label{tab:result_loc}
\vspace{-1em}
\end{table}

\begin{table}[t]
\small
\centering
\setlength{\tabcolsep}{4pt}
\begin{tabular}{c|cc}
\toprule
Model & Accuracy & Example-F1
\\ \midrule
CLIP & 0.46 & 39.90 \\
CLIP+ & 1.00 & \textbf{43.09} \\
CLIP+WIT & \textbf{1.07} & 41.73 \\
CLIP+Seg & 0.92 & 42.82 \\
\midrule
Human & 75.86 & 91.63 \\
\bottomrule
\end{tabular}
\vspace{-0.5em}\caption{Summary of the performance for different baselines on the image time prediction. Accuracy does not consider hierarchies and Example-F1 considers hierarchies.(\%)}
\label{tab:result_loc}
\vspace{-1em}
\end{table}

==> sections/6-exp.tex <==
\section{Experiments}

==> sections/sketch.tex <==
\section{Introduction Ben's Ver}

Vision and language are two of most important information sources, and the fact that humans can perform join reasoning with both sources at the same time has motivated artificial intelligence research to consider visually-grounded language understanding. Most existing related work focus on vision-language reasoning under the assumption with local evidences, \cite{suhr2018corpus, hudson2019gqa}, yet few of them break such confinement and encourage open-ended reasoning where a model needs to look beyond task inputs. This is an important aspect because humans can relate visual cues to corresponding contextual information that often exists as texts. For example, as \Cref{fig:new_york_example} shows, people that are familiar with the news can infer the location being the times square through the iconic screen panels, and further estimate the period of time through the crowds and signs. All of this can be done without including the related news pieces as inputs. In fact, even though some people cannot identify the related events through prior knowledge, they would have good intuition on how they can find textual evidences, through languages, entity names, building styles and more. In this work, we identify and formulate this problem, namely spatiotemporal grounding of images, a task to find given photos' taken time and location. This task motivates vision-language joint reasoning to a new level, as it requires open-ended reasoning based on world knowledge and common sense. 

Specifically, we propose a novel dataset \modelname{}, a challenging but valuable task that asks models to ground images to real-world spatial and temporal information. If models can accurately find such images' creation time and location, they would need to successfully link the visual clues with contexts, which are often only found in texts such as news, stories and encyclopedias. As a result, this task motivates models to consider the association between vision and language more closely and in a more open-ended setting. \Cref{fig:modi_board} shows an example of \modelname{}, and \cref{fig:india_example2} shows a possible way for a model to ground the image to its spatiotemporal information. Specifically, the system starts with grounding multiple segments from the image, and use the information to conduct a constrained search in a large news-base, until it locates specific textual information related to the image. 
